Third-Count False Acceptance in Small-Parameter VLMs: Diagnosis, Calibration, and Recovery Limits

A small-parameter vision-language model can miscount an image and independently endorse a third quantity that differs from both its open count and the annotation. We diagnose this error, third-count false acceptance (TCFA), through five relations among annotated, open, and proposed counts. Across six open-weight checkpoints in four model families, nearly identical balanced accuracy can conceal sharply different acceptance profiles. We measure paired recovery ($J_{43}$) as joint acceptance of the annotation and rejection of the frozen Base counting error on the same image. On COCO-ReM Dev, calibrating Gemma-3 $q/v$ (seed 0) standard continuation at a 20% false-acceptance budget raises paired recovery from 26 to 58 of 318 images without changing scores. Across 24 paired evaluations spanning COCO-ReM Test, external TallyQA Test, two 4B models, three seeds, and two readouts, hard-positive continuation raises true acceptance, false acceptance, and third-count acceptance in every run. Under default generated decisions, paired recovery changes by +3.62 percentage points for Qwen3.5 and -5.69 for Gemma-3 on COCO-ReM Test (with false acceptance up by 4.06 and 26.16 points), and by -0.53 and -14.50 points on TallyQA Test (with false acceptance up by 1.68 and 15.47 points). Transferring locked Dev 20% FAR thresholds to seed-0 Test sequence scores eliminates Qwen3.5's COCO-ReM advantage (-0.19 points at approximately 18% FAR) while raising Gemma-3's TallyQA recovery on standard continuation by +21.08 points (25 to 103 of 370). Even among images passing $J_{43}$, 36%-62% after calibration (and 43%-87% under default generation) still endorse at least one third wrong count, showing why paired recovery and TCFA must be evaluated alongside false acceptance.

==> evidence/base_rows.tex <==
Qwen2.5 & GR & 30.80 & 7.03 & 21.21 & 57.09 & 2.45 \\
Qwen2.5 & IR & 30.80 & 4.97 & 17.60 & 56.31 & 1.18 \\
Qwen3 & GR & 36.60 & 7.08 & 32.20 & 62.56 & 1.63 \\
Qwen3 & IR & 36.60 & 4.77 & 28.60 & 61.92 & 0.76 \\
Qwen3.5 & GR & 36.40 & 5.64 & 25.80 & 60.08 & 1.76 \\
Qwen3.5 & IR & 36.40 & 8.92 & 31.40 & 61.24 & 3.91 \\
Gemma-3 & GR & 32.00 & 48.29 & 64.80 & 58.25 & 43.16 \\
Gemma-3 & IR & 32.00 & 44.97 & 62.80 & 58.91 & 38.45 \\
Phi-3.5 & GR & 29.60 & 52.82 & 73.00 & 60.09 & 51.93 \\
Phi-3.5 & IR & 29.60 & 76.97 & 89.20 & 56.11 & 77.98 \\
LFM2.5 & GR & 38.80 & 42.00 & 73.80 & 65.90 & 41.34 \\
LFM2.5 & IR & 38.80 & 21.74 & 53.40 & 65.83 & 14.18 \\


==> evidence/budget_rows.tex <==
Qwen3.5 & 0 & 10 & 73/309 (9.79) & 72/309 (9.74) & 72/309 (9.64) & -0.32 [-1.71, 1.00] & -0.32 [-1.66, 0.98] \\
Qwen3.5 & 0 & 20 & 114/309 (19.33) & 122/309 (19.69) & 117/309 (19.44) & +2.59 [0.58, 4.90] & +0.97 [-0.99, 2.88] \\
Qwen3.5 & 0 & 40 & 132/309 (33.49) & 146/309 (33.59) & 138/309 (32.87) & +4.53 [1.33, 7.67] & +1.94 [-0.63, 4.49] \\
Qwen3.5 & 1 & 10 & 66/309 (9.85) & 63/309 (9.38) & -- & -0.97 [-2.93, 0.94] & -- \\
Qwen3.5 & 1 & 20 & 107/309 (19.90) & 110/309 (18.97) & -- & +0.97 [-1.26, 3.37] & -- \\
Qwen3.5 & 1 & 40 & 132/309 (34.92) & 131/309 (34.56) & -- & -0.32 [-3.13, 2.36] & -- \\
Qwen3.5 & 2 & 10 & 63/309 (9.79) & 66/309 (9.85) & -- & +0.97 [-0.64, 2.74] & -- \\
Qwen3.5 & 2 & 20 & 112/309 (19.64) & 115/309 (19.69) & -- & +0.97 [-0.92, 2.76] & -- \\
Qwen3.5 & 2 & 40 & 134/309 (34.15) & 130/309 (34.36) & -- & -1.29 [-2.96, 0.00] & -- \\
Gemma-3 $q/k/v$ & 0 & 10 & 44/318 (9.18) & 36/318 (9.74) & 37/318 (9.49) & -2.52 [-4.97, 0.00] & -2.20 [-4.53, 0.00] \\
Gemma-3 $q/k/v$ & 0 & 20 & 62/318 (19.69) & 56/318 (19.69) & 55/318 (18.62) & -1.89 [-4.69, 0.97] & -2.20 [-4.79, 0.32] \\
Gemma-3 $q/k/v$ & 0 & 40 & 59/318 (29.13) & 54/318 (25.64) & 70/318 (26.97) & -1.57 [-4.81, 1.58] & +3.46 [0.61, 6.77] \\


==> evidence/calibration_rows.tex <==
Qwen3.5 & 10 & 115/309 & 73/309 & 20.97 & 9.79 & -13.59 [-18.10, -9.03] \\
Qwen3.5 & 20 & 115/309 & 114/309 & 20.97 & 19.33 & -0.32 [-1.99, 1.30] \\
Qwen3.5 & 40 & 115/309 & 132/309 & 20.97 & 33.49 & +5.50 [0.65, 10.38] \\
Gemma-3 $q/k/v$ & 10 & 34/318 & 44/318 & 60.26 & 9.18 & +3.14 [-1.94, 8.09] \\
Gemma-3 $q/k/v$ & 20 & 34/318 & 62/318 & 60.26 & 19.69 & +8.81 [3.57, 14.33] \\
Gemma-3 $q/k/v$ & 40 & 34/318 & 59/318 & 60.26 & 29.13 & +7.86 [3.07, 12.63] \\


==> evidence/ranking_rows.tex <==
Qwen3.5 & A & 0.6574 & 218/309 & 0 & +0.0000 & +0.0000 \\
Qwen3.5 & D & 0.6709 & 219/309 & 0 & +0.1877 & +0.0032 \\
Qwen3.5 & E & 0.6653 & 220/309 & 0 & +0.1316 & -0.0008 \\
Gemma-3 $q/k/v$ & A & 0.4532 & 160/318 & 0 & +0.0000 & +0.0000 \\
Gemma-3 $q/k/v$ & D & 0.4536 & 165/318 & 0 & +0.5625 & +0.0000 \\
Gemma-3 $q/k/v$ & E & 0.4590 & 168/318 & 0 & +0.3750 & +0.0000 \\


==> evidence/relation_rows.tex <==
Qwen2.5 & GR & 60.40 (149) & 5.94 (572) & 35.58 (208) & 4.55 (330) & 2.45 (1104) \\
Qwen2.5 & IR & 51.30 (154) & 4.36 (573) & 27.27 (209) & 2.73 (330) & 1.18 (1104) \\
Qwen3 & GR & 74.86 (183) & 6.40 (688) & 38.50 (200) & 7.67 (313) & 1.63 (1046) \\
Qwen3 & IR & 69.40 (183) & 4.22 (688) & 28.00 (200) & 5.11 (313) & 0.76 (1046) \\
Qwen3.5 & GR & 62.09 (182) & 7.88 (685) & 18.36 (207) & 5.18 (309) & 1.76 (1022) \\
Qwen3.5 & IR & 70.88 (182) & 11.82 (685) & 25.12 (207) & 9.06 (309) & 3.91 (1022) \\
Gemma-3 & GR & 86.25 (160) & 48.82 (594) & 71.76 (216) & 55.66 (318) & 43.16 (1038) \\
Gemma-3 & IR & 86.25 (160) & 48.26 (605) & 68.98 (216) & 52.83 (318) & 38.45 (1043) \\
Phi-3.5 & GR & 95.95 (148) & 41.26 (555) & 88.46 (208) & 63.40 (347) & 51.93 (1167) \\
Phi-3.5 & IR & 98.65 (148) & 67.93 (555) & 95.19 (208) & 85.30 (347) & 77.98 (1167) \\
LFM2.5 & GR & 97.94 (194) & 29.04 (730) & 93.26 (193) & 58.11 (296) & 41.34 (987) \\
LFM2.5 & IR & 92.27 (194) & 17.26 (730) & 80.83 (193) & 29.39 (296) & 14.18 (987) \\


==> evidence/sft_rows.tex <==
Base & GR & 36.40 & 25.80 & 5.64 & 60.08 & 1.76 \\
Joint SFT & GR & 45.20 & 51.00 & 17.38 & 66.81 & 10.72 \\
Base & IR & 36.40 & 31.40 & 8.92 & 61.24 & 3.91 \\
Joint SFT & IR & 45.20 & 48.80 & 16.77 & 66.02 & 9.09 \\


==> evidence/state_rows.tex <==
Qwen3.5 & A & 109 & 59 & 115 & 26 & 114 & 59 & 114 & 22 \\
Qwen3.5 & D & 95 & 59 & 123 & 32 & 113 & 56 & 122 & 18 \\
Qwen3.5 & E & 97 & 59 & 121 & 32 & 114 & 58 & 117 & 20 \\
Gemma-3 $q/k/v$ & A & 17 & 45 & 34 & 222 & 131 & 77 & 62 & 48 \\
Gemma-3 $q/k/v$ & D & 5 & 22 & 12 & 279 & 128 & 78 & 56 & 56 \\
Gemma-3 $q/k/v$ & E & 7 & 30 & 16 & 265 & 133 & 80 & 55 & 50 \\

